Toric differential forms and periods of complete intersections

Let $n$ be an even natural number. We compute the periods of any $\frac{n}{2}$-dimensional complete intersection algebraic cycle inside an $n$-dimensional non-degenerated intersection of a projective simplicial toric variety. Using this information we determine the cycle class of such algebraic cycles. As part of the proof we develop a toric generalization of a classical theorem of Macaulay about complete intersection Artin Gorenstein rings, and we generalize an algebraic cup formula for residue forms due to Carlson and Griffiths to the toric setting.

==> s12.tex <==
Let us introduce an Artinian Gorenstein ideal associated to a Hodge cycle of a quasi-smooth hypersurface $X\subseteq\P_\Sigma$.

\begin{dfn}
Let $\P_\Sigma$ be an $m$-dimensional projective simplicial toric variety and $X=\{F=0\}\subseteq \P_\Sigma$ be a quasi-smooth hypersurface of even dimension $n=m-1$, corresponding to an ample divisor with $\deg(F)=\beta\in\Cl(\P_\Sigma)$. Let $\lambda\in H^{\frac{n}{2},\frac{n}{2}}(X)_\prim\cap H^n(X,\Q)$ be a non-trivial primitive Hodge class with Poincar\'e dual the homology cycle $\lambda^\pd=\delta\in H_n(X,\Q)$. The \textit{Artinian Gorenstein ideal associated to $\lambda$} is the homogeneous ideal of the Cox ring $S(\Sigma)$ given by
$$
J(\lambda)^\alpha:=\left\{P\in S(\Sigma)^\alpha: \int_\delta \res\left(\frac{PQ\Omega}{F^{\frac{n}{2}+1}}\right)=0 \ , \ \ \forall Q\in S(\Sigma)^{N-\alpha}\right\}
$$
where $N:=(\frac{n}{2}+1)\beta-\beta_0$ and $\beta_0$ is the anti-canonical class.
\end{dfn}

\begin{rmk}
By definition $J(\lambda)$ is Artinian Gorenstein of socle in degree $N$. In other words all the degrees $\alpha\in\Cl(\P_\Sigma)$ are regular for $(J(\lambda),N)$.
\end{rmk}

\begin{thm}
\label{theoideals}
Let $\P_\Sigma$ be an $m$-dimensional projective simplicial toric variety and $X=\{F=0\}\subseteq\P_\Sigma$ be a non-degenerated hypersurface of even dimension $n=m-1$, corresponding to an ample divisor with $\deg(F)=\beta\in\Cl(\P_\Sigma)$. Consider the (not necessarily quasi-smooth) complete intersection subvariety
$$
Z:=\{g_1=g_2=\cdots=g_{\frac{n}{2}+1}=0\}\subseteq\P_\Sigma
$$
such that $Z\subseteq X$. Let $N:=(\frac{n}{2}+1)\beta-\beta_0$ where $\beta_0$ is the anti-canonical class. Then
$$
J(\eta_Z)^N=\langle g_1,h_1,\ldots,g_{\frac{n}{2}+1},h_{\frac{n}{2}+1}\rangle^N=(J_1(F):P_Z)^N
$$
where $F=g_1\cdot h_1+\cdots+g_{\frac{n}{2}+1}\cdot h_{\frac{n}{2}+1}$ and $P_Z$ is given by \cref{mainthm}.
\end{thm}

\begin{proof}
Note first that by definition $N$ is a socle degree for $J(\eta_Z)$. By \cref{teomactor} it is also a socle degree for $I:=\langle g_1,h_1,\ldots,g_{\frac{n}{2}+1},h_{\frac{n}{2}+1}\rangle$. By \cref{corunimodj1} and \cref{propcoxgor} we know $N$ is also a socle degree for $(J_1(F):P_Z)$. Noting that $\res\left(\frac{g_iQ\Omega}{F^{\frac{n}{2}+1}}\right)|_Z\equiv 0$ it follows that each $g_i\in J(\eta_Z)$. On the other hand, if we let
$$
Z_i:=\{g_1=\cdots=g_{i-1}=h_i=g_{i+1}=\cdots=g_{\frac{n}{2}+1}=0\}\subseteq\P_\Sigma
$$
then $\eta_Z+\eta_{Z_i}=0\in H^{\frac{n}{2},\frac{n}{2}}(X)_\prim$, thus
$$
\int_Z\res\left(\frac{h_iQ\Omega}{F^{\frac{n}{2}+1}}\right)=-\int_{Z_i}\res\left(\frac{h_iQ\Omega}{F^{\frac{n}{2}+1}}\right)=0
$$
and so $h_i\in J(\eta_Z)$. This shows the first equality $J(\eta_Z)^N=I^N$. For the second one we use the explicit description of $P_Z$ given in \cref{mainthm} to check that
$$
P_Z\cdot x_1\cdots x_r=\frac{(-1)^{sgn(\sigma)}\frac{n}{2}!x_{\rho_1}\cdots x_{\rho_{n+1}}x_{\rho_\ell}}{k_\ell\det(\rho_1|\cdots|\rho_{n+1})^2}\det\begin{pmatrix}\frac{\partial g_1}{\partial x_{\rho_\ell}} & \frac{\partial h_1}{\partial x_{\rho_\ell}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} \\ \frac{\partial g_1}{\partial x_{\rho_1}} & \frac{\partial h_1}{\partial x_{\rho_1}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_1}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_1}}\\
\vdots & \vdots &  & \vdots & \vdots \\
\frac{\partial g_1}{\partial x_{\rho_{n+1}}} & \frac{\partial h_1}{\partial x_{\rho_{n+1}}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_{n+1}}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_{n+1}}} \end{pmatrix}
$$
then if $c_\ell:=\frac{(-1)^{sgn(\sigma)}\frac{n}{2}!}{k_\ell\det(\rho_1|\cdots|\rho_{n+1})^2}$, then
$$
g_1\cdot P_Z\cdot x_1\cdots x_r=c_\ell\cdot x_{\rho_1}\cdots x_{\rho_m}x_{\rho_\ell}\det\begin{pmatrix}\frac{\partial g_1}{\partial x_{\rho_\ell}} & g_1\frac{\partial h_1}{\partial x_{\rho_\ell}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} \\ \frac{\partial g_1}{\partial x_{\rho_1}} & g_1\frac{\partial h_1}{\partial x_{\rho_1}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_1}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_1}}\\
\vdots & \vdots &  & \vdots & \vdots \\
\frac{\partial g_1}{\partial x_{\rho_m}} & g_1\frac{\partial h_1}{\partial x_{\rho_m}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_m}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_m}} \end{pmatrix}
$$
$$
=c_\ell\cdot x_{\rho_1}\cdots x_{\rho_m}x_{\rho_\ell}\det\begin{pmatrix}\frac{\partial g_1}{\partial x_{\rho_\ell}} & \frac{\partial F}{\partial x_{\rho_\ell}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} \\ \frac{\partial g_1}{\partial x_{\rho_1}} & \frac{\partial F}{\partial x_{\rho_1}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_1}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_1}}\\
\vdots & \vdots &  & \vdots & \vdots \\
\frac{\partial g_1}{\partial x_{\rho_m}} & \frac{\partial F}{\partial x_{\rho_m}} & \cdots & \frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_m}} & \frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_m}} \end{pmatrix}
$$
$$
=c_\ell\cdot\det\begin{pmatrix}x_{\rho_\ell}\frac{\partial g_1}{\partial x_{\rho_\ell}} & x_{\rho_\ell}\frac{\partial F}{\partial x_{\rho_\ell}} & \cdots & x_{\rho_\ell}\frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} & x_{\rho_\ell}\frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_\ell}} \\ x_{\rho_1}\frac{\partial g_1}{\partial x_{\rho_1}} & x_{\rho_1}\frac{\partial F}{\partial x_{\rho_1}} & \cdots & x_{\rho_1}\frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_1}} & x_{\rho_1}\frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_1}}\\
\vdots & \vdots &  & \vdots & \vdots \\
x_{\rho_m}\frac{\partial g_1}{\partial x_{\rho_m}} & x_{\rho_m}\frac{\partial F}{\partial x_{\rho_m}} & \cdots & x_{\rho_m}\frac{\partial g_{\frac{n}{2}+1}}{\partial x_{\rho_m}} & x_{\rho_m}\frac{\partial h_{\frac{n}{2}+1}}{\partial x_{\rho_m}} \end{pmatrix}\in J_0(F).
$$
In other words $g_1\in (J_0(F):P_Z\cdot x_1\cdots x_r)=(J_1(F):P_Z)$. Similarly one sees that all $g_i,h_i\in (J_1(F):P_Z)$ and so $I^N=(J_1(F):P_Z)^N$.
\end{proof}

==> s15.tex <==
\begin{thm}
Let $\P_\Sigma$ be a $d$-dimensional projective simplicial toric variety and $X\subseteq \P_\Sigma$ be an $n$-dimensional quasi-smooth intersection of ample hypersurfaces, with $n$ even. Then every (not necessarily quasi-smooth) complete intersection algebraic cycle $Z\in \CH^\frac{n}{2}(X)$ satisfies the variational Hodge conjecture and $V_{[Z]}$ is smooth. Furthermore, the locus 
$$
T_{(\alpha_1,\ldots,\alpha_\frac{d+s}{2})}:=\left\{t\in T: \begin{matrix}X_t\text{ contains a complete intersection cycle} \\
\text{defined by }\deg(g_i)=\alpha_i\in\Cl(\P_\Sigma)\end{matrix}\right\}
$$
is a component of $\HL_{(\beta_1,\ldots,\beta_s)}(\P_\Sigma)$.
\end{thm}

... In order to prove this result, we need to show that $\beta$ is regular for $(I,N)$ where $I=\langle g_1,h_1,\ldots,g_\frac{d+s}{2},h_\frac{d+s}{2}\rangle$ and $N=(\frac{d+s}{2})\beta-\beta_0$. In order to do this try to adapt the proof of \cite{mustata2002vanishing}...
